Fast sensor placement by enlarging principle submatrix for large-scale linear inverse problems

Sensor placement for linear inverse problems is the selection of locations to assign sensors so that the entire physical signal can be well recovered from partial observations. In this paper, we propose a fast sampling algorithm to place sensors. Specifically, assuming that the field signal $\mathbf{f}$ is represented by a linear model $\mathbf{f}=\pmb{\phi}\mathbf{g}$, it can be estimated from partial noisy samples via an unbiased least-squares (LS) method, whose expected mean square error (MSE) depends on chosen samples. First, we formulate an approximate MSE problem, and then prove it is equivalent to a problem related to a principle submatrix of $\pmb{\phi}\pmb{\phi}^\top$ indexed by sample set. To solve the formulated problem, we devise a fast greedy algorithm with simple matrix-vector multiplications, leveraging a matrix inverse formula. To further reduce complexity, we reuse results in the previous greedy step for warm start, so that candidates can be evaluated via lightweight vector-vector multiplications. Extensive experiments show that our proposed sensor placement method achieved the lowest sensor sampling time and the best performance compared to state-of-the-art schemes.

==> gda.tex <==
\section{Gershgorin Disc Alignment}

Denote by $\bPhi_{\bS_t}$ the matrix with rows and columns indexed by set $\bS_t$.
In the next iteration, the newly chosen submatrix is $\bPhi_{\bS_{t+1}}$, where $\bS_{t+1} = \bS_t \setminus \{k\}$ and $k$ is the index of the chosen row / column to be removed from $\bPhi_{\bS_t}$.
At each iteration $t$, the goal is to select index $k$ such that the condition number of $\bPhi_{\bS_{t+1}}$ is minimized.

From GCT, a lower bound $\lambda_{\min}^-$ of $\lambda_{\min}(\bPhi_{\bS_{t+1}})$ can be computed as
\begin{align}
\lambda_{\min}^- = \min_{i \in \bS_{t+1}}
\bPhi_{\bS_{t+1}}(i,i) - \sum_{k \in \bS_{t+1} | k \neq i} |\bPhi_{\bS_{t+1}}(i,k)|
\label{eq:GCT_lower}
\end{align}
This lower bound $\lambda_{\min}^-$ is in general loose.
In \red{cite Cheng's PAMI submission}, it is proven that using the first eigenvector $\v$ of $\bPhi_{\bS_{t+1}}$, one can compute a diagonal matrix $\Q = \text{diag}(1/v_1, 1/v_2, \ldots)$, so that similar transform $\bTheta_{\bS_{t+1}} = \Q \bPhi_{\bS_{t+1}} \Q^{-1}$ of $\bPhi_{\bS_{t+1}}$ has its Gershgorin disc left-ends perfectly aligned at $\lambda_{\min}(\bTheta_{\bS_{t+1}}) = \lambda_{\min}(\bPhi_{\bS_{t+1}})$.
This means that the lower bound $\lambda^-_{\min}$ computed using \eqref{eq:GCT_lower} for $\bTheta_{\bS_{t+1}}$ is as tight as possible.

Of course, computing $\v$ for each $\bPhi_{\bS_{t+1}}$ corresponding to candidate index $k$ is too computation expensive.
Thus, we develop the following strategy.
We first note that, due to Cauchy's interlace theorem, $\lambda_{\min}$ of submatrix $\bPhi_{\bS_{t+1}}$ is no smaller than the larger matrix $\bPhi_{\bS_{t}}$, \textit{i.e.},
\begin{align}
\lambda_{\min}(\bPhi_{\bS_{t}}) \leq \lambda_{\min}(\bPhi_{\bS_{t+1}})
\end{align}

Second, suppose we first perform similar transform on $\bPhi_{\bS_{t}}$ to arrive at $\bTheta_{\bS_{t}}$, then select row/column index $k$ with the largest corresponding $\lambda^-_{\min}(\bTheta_{\bS_{t+1}})$.
We know that $\lambda_{\min}(\bPhi_{\bS_{t}}) \leq \lambda^-_{\min}(\bTheta_{\bS_{t+1}})$, since we are eliminating one entire row $k$ and one element in each of the remaining rows in $\bTheta_{\bS_{t}}$, and hence the disc radius in row $j \neq k$ of new $\bTheta_{\bS_{t+1}}$ will be no larger.
Thus the GCT bound for candidate $k$ is at least as good as $\lambda_{\min}(\bPhi_{\bS_{t}})$, which would not be the case of we greedily choose an index from $\bPhi_{\bS_{t}}$ directly instead of similar transform $\bTheta_{\bS_{t}}$.
